Unreachability of $\bf{\Gamma_{2n+1,m}}$

We find bounds for the maximal length of a sequence of distinct $\bf{\Gamma_{2n+1,m}}$-sets under $AD$ and show there is no sequence of distinct $\bf{\Gamma_{2n+1}}$-sets of length $\bf{\delta^1_{2n+3}}$. As a special case, there is no sequence of distinct $\bf{\Gamma_{1,m}}$-sets of length $\aleph_{m+2}$. These are the optimal results for the pointclasses $\bf{\Gamma_{2n+1}}$ and $\bf{\Gamma_{1,m}}$.

==> bib.tex <==
@article{twoapp,
 author = {Greg Hjorth},
 journal = {The Bulletin of Symbolic Logic},
 number = {1},
 pages = {94--107},
 publisher = {[Association for Symbolic Logic, Cambridge University Press]},
 title = {Two Applications of Inner Model Theory to the Study of $\bf{\Sigma^1_2}$ Sets},
 volume = {2},
 year = {1996}
}

@misc{hra,
  doi = {10.48550/ARXIV.2105.06403},
  
  url = {https://arxiv.org/abs/2105.06403},
  
  author = {Sargsyan, Grigor},
  
  keywords = {Logic (math.LO), FOS: Mathematics, FOS: Mathematics},
  
  title = {Hjorth's Reflection Argument},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {Creative Commons Attribution Non Commercial Share Alike 4.0 International}
}

@Inbook{Neeman2010,
author="Neeman, Itay",
editor="Foreman, Matthew
and Kanamori, Akihiro",
title="Determinacy in L($\mathbb{R}$)",
bookTitle="Handbook of Set Theory",
year="2010",
publisher="Springer Netherlands",
address="Dordrecht",
pages="1877--1950",
url="https://doi.org/10.1007/978-1-4020-5764-9_23"
}

@InProceedings{scales,
author="Steel, John R.",
editor="Kechris, Alexander S.
and Martin, Donald A.
and Moschovakis, Yiannis N.",
title="Scales in L(R)",
booktitle="Cabal Seminar 79--81",
year="1983",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="107--156",
isbn="978-3-540-38680-3"
}

@incollection{Kechris,
title = {On Transfinite Sequences of Projective Sets with an Application to $\Sigma^1_2$ Equivalence Relations},
editor = {Angus Macintyre and Leszek Pacholski and Jeff Paris},
series = {Studies in Logic and the Foundations of Mathematics},
publisher = {Elsevier},
volume = {96},
pages = {155-160},
year = {1978},
booktitle = {Logic Colloquium '77},
author = {Alexander S. Kechris}
}

@article{Harrington,
 author = {Leo Harrington},
 journal = {The Journal of Symbolic Logic},
 number = {4},
 pages = {685--693},
 publisher = {[Association for Symbolic Logic, Cambridge University Press]},
 title = {Analytic Determinacy and $0^\#$},
 volume = {43},
 year = {1978}
}

@article{Jackson,
title = {Partition properties and well-ordered sequences},
journal = {Annals of Pure and Applied Logic},
volume = {48},
number = {1},
pages = {81-101},
year = {1990},
author = {Steve Jackson}
}

@unpublished{cmi,
title = {The Core Model Induction},
author = {Ralf Schindler and John Steel},
url = {https://ivv5hpp.uni-muenster.de/u/rds/core_model_induction.pdf}
}

@inbook{hacm, place={Cambridge}, series={Lecture Notes in Logic}, title={HOD as a core model}, volume={3}, DOI={10.1017/CBO9781139519694.010}, booktitle={Ordinal Definability and Recursion Theory: The Cabal Seminar, Volume III}, publisher={Cambridge University Press}, author={Steel, John R. and Woodin, W. Hugh}, editor={Kechris, Alexander S. and Löwe, Benedikt and Steel, John R.}, year={2016}, pages={257–346}, collection={Lecture Notes in Logic}}

@inbook{steel2016, place={Cambridge}, series={Lecture Notes in Logic}, title={A theorem of Woodin on mouse sets}, volume={3}, DOI={10.1017/CBO9781139519694.009}, booktitle={Ordinal Definability and Recursion Theory: The Cabal Seminar, Volume III}, publisher={Cambridge University Press}, author={Steel, John R.}, editor={Kechris, Alexander S. and Löwe, Benedikt and Steel, John R.}, year={2016}, pages={243–256}, collection={Lecture Notes in Logic}}

@book{mosdst,
author = {Yiannis Moschovakis},
title = {Descriptive Set Theory},
series = {Mathematical surveys and monographs; no. 155},
publisher = {American Mathematical Society},
year = {2009},
isbn = {978-1-4704-1382-8}}

@article{self-iter,
 author = {Ralf Schindler and John Steel},
 journal = {The Journal of Symbolic Logic},
 number = {3},
 pages = {751--779},
 publisher = {[Association for Symbolic Logic, Cambridge University Press]},
 title = {The Self-Iterability of L[E]},
 volume = {74},
 year = {2009}
}

@book{msbook, place={Cambridge}, series={Lecture Notes in Logic}, title={Fine Structure and Iteration Trees}, DOI={10.1017/9781316718315}, publisher={Cambridge University Press}, author={Mitchell, William J. and Steel, John R.}, year={2017}, collection={Lecture Notes in Logic}}

@misc{sihmor,
  doi = {10.48550/ARXIV.1210.7258},
  url = {https://arxiv.org/abs/1210.7258},
  author = {Schlutzenberg, Farmer and Trang, Nam},
  keywords = {Logic (math.LO), FOS: Mathematics, FOS: Mathematics, 03E45, 03E60, 03E15},
  title = {Scales in hybrid mice over $\mathbb{R}$},
  publisher = {arXiv},
  year = {2012},
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@Inbook{ooimt,
author="Steel, John R.",
editor="Foreman, Matthew
and Kanamori, Akihiro",
title="An Outline of Inner Model Theory",
bookTitle="Handbook of Set Theory",
year="2010",
publisher="Springer Netherlands",
address="Dordrecht",
pages="1595--1684",
}

@article{dmatm,
author = {Steel, John},
year = {2008},
month = {05},
pages = {},
title = {Derived models associated to mice},
volume = {14},
isbn = {978-981-279-653-0},
journal = {Lect. Notes Ser. Inst. Math. Sci. Natl. Univ. Singap.},
doi = {10.1142/9789812794055_0003}
}

@article{hodbelowtheta,
 ISSN = {10798986},
 URL = {http://www.jstor.org/stable/420947},
 author = {John R. Steel},
 journal = {The Bulletin of Symbolic Logic},
 number = {1},
 pages = {75--84},
 publisher = {[Association for Symbolic Logic, Cambridge University Press]},
 title = {$HOD^{L(R)}$ Is a Core Model below $\Theta$},
 urldate = {2022-10-14},
 volume = {1},
 year = {1995}
}

@inbook{jackson_2011, place={Cambridge}, series={Lecture Notes in Logic}, title={AD and the Projective Ordinals}, booktitle={Wadge Degrees and Projective Ordinals: The Cabal Seminar, Volume II}, publisher={Cambridge University Press}, author={Jackson, Steve}, editor={Kechris, Alexander S. and Löwe, Benedikt and Steel, John R.Editors}, year={2011}, pages={364–483}, collection={Lecture Notes in Logic}}

@inbook{largest_ctble, place={Cambridge}, series={Lecture Notes in Logic}, title={The Largest Countable This, That, and the Other}, booktitle={Games, Scales and Suslin Cardinals: The Cabal Seminar, Volume I}, publisher={Cambridge University Press}, author={Martin, Donald A.}, editor={Kechris, Alexander S. and Löwe, Benedikt and Steel, John R.Editors}, year={2008}, pages={121–129}, collection={Lecture Notes in Logic}}

@article{optimal_det, title={Optimal Proofs of Determinacy}, volume={1}, number={3}, journal={Bulletin of Symbolic Logic}, publisher={Cambridge University Press}, author={Neeman, Itay}, year={1995}, pages={327–339}}

@article{bddness_lemma, title={A Boundedness Lemma for Iterations}, volume={66}, number={3}, journal={The Journal of Symbolic Logic}, publisher={Cambridge University Press}, author={Hjorth, Greg}, year={2001}, pages={1058–1072}}

@article{on_the_pwo,
 author = {Sargsyan, Grigor},
 journal = {The Journal of Symbolic Logic},
 number = {3},
 pages = {735--763},
 publisher = {[Association for Symbolic Logic, Cambridge University Press]},
 title = {On The Prewellorderings Associated with the Directed Systems of Mice},
 volume = {78},
 year = {2013}
}

@phdthesis{phdthesis,
  author       = {Derek Levinson}, 
  title        = {Unreachability of Inductive-Like Pointclass in $L(\mathbb{R})$},
  school       = {University of California, Los Angeles},
  year         = 2023,
}

@article{pwoim,
title = {Projectively Well-ordered Inner Models},
journal = {Annals of Pure and Applied Logic},
volume = {74},
number = {1},
pages = {77-104},
year = {1995},
author = {J.R. Steel}
}
